Statistical Inference under Performativity

Performativity of predictions refers to the phenomenon where prediction-informed decisions influence the very targets they aim to predict -- a dynamic commonly observed in policy-making, social sciences, and economics. In this paper, we initiate an end-to-end framework of statistical inference under performativity. Our contributions are twofold. First, we establish a central limit theorem for estimation and inference in the performative setting, enabling standard inferential tasks such as constructing confidence intervals and conducting hypothesis tests in policy-making contexts. Second, we leverage this central limit theorem to study prediction-powered inference (PPI) under performativity. This approach yields more precise estimates and tighter confidence regions for the model parameters (i.e., policies) of interest in performative prediction. We validate the effectiveness of our framework through numerical experiments. To the best of our knowledge, this is the first work to establish a complete statistical inference under performativity, introducing new challenges and inference settings that we believe will provide substantial value to policy-making, statistics, and machine learning.

==> Sections/related_works.tex <==
\paragraph{Performative prediction.} Performativity describes the phenomenon whereby predictions influence the outcomes they aim to predict. \cite{perdomo2020performative} were the first to formalize performative prediction in the supervised‐learning setting; their work, along with the majority of subsequent papers \citep{MendlerDnner2020StochasticOF, Drusvyatskiy2020StochasticOW, Mofakhami2023PerformativePW, Oesterheld2023IncentivizingHP, Taori2022DataFL, Khorsandi2024TightLB, Perdomo2025RevisitingTP，bracale2024microfoundation}, have been focused on performative stability and proposed algorithms for learning performative stable parameters. On the other hand, performative optimality requires much stricter conditions (e.g. distributional assumptions to ensure the convexity of $\text{PR}(\theta)$) than performative stability, a few papers address the problem of finding performative optimal parameters. \cite{Miller2021OutsideTE} introduce a two‐stage method that learns a distribution map to locate the performative optimal parameter. \cite{Kim2022MakingDU} study performative optimality in outcome‐only performative settings. Finally, \cite{Hardt2023PerformativePP} provide a comprehensive overview of learning algorithms, optimization methods, and applications for performative prediction. Unlike these prior works on performative prediction, which focus on prediction accuracy, our work is dedicated to constructing powerful and statistically valid inference procedures under the performative framework.

\paragraph{Prediction-powered inference.} \cite{Angelopoulos2023PredictionpoweredI} first introduced the prediction-powered inference (PPI) framework, which leverages black-box machine learning models to construct valid confidence intervals (CIs) for statistical quantities. Since then, PPI has been extended and applied in various settings. Closely related to our strategies, \cite{angelopoulos2023ppi++} propose PPI++, a more computationally efficient procedure that enhances predictability by accommodating a wider range of models on unlabeled data, while guaranteeing performance (e.g.\ CI width) no worse than that of classical inference methods. Other extensions include Stratified PPI \citep{Fisch2024StratifiedPI}, which incorporates simple data stratification strategies into basic PPI estimates; Cross PPI \citep{Zrnic2023CrosspredictionpoweredI}, which obtain confidence intervals with significantly lower variability by including model training; Bayesian PPI \citep{Hofer2024BayesianPI} and FAB-PPI \citep{Cortinovis2025FABPPIFA}, which propose frameworks for PPI based on Bayesian inference. PPI is also connected to topics such as semi-parametric inference and missing-data imputation \citep{Tsiatis2006SemiparametricTA,Robins1995SemiparametricEI,Demirtas2018FlexibleIO,Song2023AGM}. Our work is the first one to study PPI under performativity, and we validate the PPI framework in the performative setting both theoretically and empirically.

==> Sections/setup.tex <==
\section{Setup}
We mainly consider the repeated risk minimization setting. At time $t=0$, we have access to a set of labeled data $\{z_{0,i}\}_{i=1}^{n_0}$ that is i.i.d. drawn from a distribution $\cD(\theta_0)$, where $z_{0,i}=(x_{0,i},y_{0,i})$ and $\theta_0$ is chosen by us. Then, we use the empirical repeated risk minimization to output 
$$\hat\theta_1=\argmin_{\theta\in\Theta}\frac{1}{n_0}\sum_{i=1}^{n_0}\ell (z_{0,i};\theta)$$ as an estimator of $\theta_1=\argmin_{\theta\in\Theta}\bE_{z\sim \cD(\theta_0)}\ell(z;\theta).$
Then, for $t\ge 1$, at time $t$, we further have access to a set of labeled data $\{z_{t,i}\}_{i=1}^{n_t}$ that are i.i.d. drawn from the distribution induced by last iteration, i.e., $\cD(\hat\theta_{t})$. Let us further define $G(\tilde \theta)=\argmin_{\theta\in\Theta}\bE_{z\sim \cD(\tilde \theta)}\ell(z;\theta).$
Then, we can obtain output 
$$\hat \theta_{t+1}=\argmin_{\theta\in\Theta}\frac{1}{n_t}\sum_{i=1}^{n_t}\ell (z_{t,i};\theta)$$
as an estimator of $\theta_{t+1}=G(\theta_t)$. This iterative process will incur two trajectories. %\zhun{we should add a plot here}
\begin{itemize}
\item\textbf{Underlying trajectory:} $\theta_0\rightarrow\theta_1\rightarrow\cdots \theta_t\rightarrow  \cdots $
\item\textbf{Trajectory in practice:} $\theta_0\rightarrow\hat\theta_1\rightarrow\cdots \hat\theta_t\rightarrow  \cdots $
\end{itemize}
%Our aim is to use $\hat\theta_T$ for a certain $T$ to estimate $\theta_{\text{PS}}$ and to design a statistically principled mechanism $M$ to get a more accurate estimator of $\theta_{\text{PS}}$ i.e., providing tighter confidence region for $\hat\theta_T-\theta_{\text{PS}}$ and achieving smaller $\bE\|\hat\theta_T-\theta_{\text{PS}}\|$.

Our aim is to provide inference on $\hat \theta_t$ for any $t\ge 1$. %In particular, as we know that the trajectory $\{\theta_t\}_t$ will approximate $\theta_{\text{PS}}$ as $t$ increases, we would expect 
